MicroFuzz: An Efficient Fuzzing Framework for Microservices

This paper presents a novel fuzzing framework, called MicroFuzz, specifically designed for Microservices. Mocking-Assisted Seed Execution, Distributed Tracing, Seed Refresh and Pipeline Parallelism approaches are adopted to address the environmental complexities and dynamics of Microservices and improve the efficiency of fuzzing. MicroFuzz has been successfully implemented and deployed in Ant Group, a prominent FinTech company. Its performance has been evaluated in three distinct industrial scenarios: normalized fuzzing, iteration testing, and taint verification.Throughout five months of operation, MicroFuzz has diligently analyzed a substantial codebase, consisting of 261 Apps with over 74.6 million lines of code (LOC). The framework's effectiveness is evident in its detection of 5,718 potential quality or security risks, with 1,764 of them confirmed and fixed as actual security threats by software specialists. Moreover, MicroFuzz significantly increased program coverage by 12.24% and detected program behavior by 38.42% in the iteration testing.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> issta_review.tex <==
ISSTA'23 Paper #409 Reviews and Comments
===========================================================================
Paper #409 RockFuzz: A Novel Fuzzing Framework for Microservices at the
Industrial Level


Review #409A
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper presents RockFuzz, a fuzzer for microservices.  RockFuzz combines various techniques to deliver a solution that is applicable to different industrial scenarios, in particular normal fuzzing, iteration testing and taint verification.  The evaluation is done on microservices from a fintech company.

Strengths
---------
- framework applicable to various industrial scenarios
- good results

Weaknesses
----------
- unclear research contributions
- some parts of the paper are not clear

Comments for authors
--------------------
RockFuzz addresses an important application domain, that of microservices testing.
The framework is shown to be applicable to three different industrial scenarios, with good overall results.

However, the research contribution seems weak overall.
RockFuzz combines existing techniques, such as combination testing, mocking point identification, directed fuzzing, software testing as species discovery, tainting, etc. in a practical system, but it is difficult to identify the research contributions it makes. 
In my opinion, the paper would be more appropriate for e.g, the ICSE SEIP track or the ISSTA tool demo track.

Many aspects are clearly described, but not all.
For instance, while discovering 1600 vulnerabilities is impressive, how do you check for false positives?  For duplicates?  How many reports were confirmed by developers?   How many were fixed?
Also, Table 2 is quite confusing: summing up the number of vulnerabilities, we get 12 vulnerabilities, so how is the total 1615?

If you tested 84 microservices, why present data for only 10?  How were those 10 selected?

To improve the presentation, the design and implementation should separated.  Right now, the design part refers to many implementation details, such as specific Java APIs, e.g., String Bean, MyBatis, etc.  In fact, the paper should make it clear from the beginning that the framework targets microservices written in Java.

Figure 2 is very hard to follow with so many edges, it should be simplified/modularised in some way.

The paper has a number of proofreading issues, some of which make the paper difficult to read.   For instance: "evaluate" (page 1 and elsewhere) should be "evolve"; "microservices has", "third libraries", "each each"; "scene" instead of "scenario"; "normalized fuzzing"; "unprecedented" (pg 6, what does it mean?), etc.

I found 4.2.1 difficult to follow, a diagram might be useful there.

Step 3 in 4.3 was also unclear.  What is "j" there?  An example might be useful.

Fuzzing decoupling, presented and evaluated in 5.1.3 and 5.1.4 is unclear and something that I would expect to be presented in the design rather than the evaluation section.

Is RockFuzz available?  Is data going to be available, at least for a subset of the microservices considered?

Questions for authors’ response
-------------------------------
- How do you process the large number of vulnerability reports and deal with false positives?
- Why report data on only 10 microservices?  How were these selected?
- What is the meaning of the total line in Table 2?
- Is RockFuzz and/or associated data available?



Review #409B
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
Most work on fuzzing focuses on a single (monolithic) application. In contrast, this work proposes a fuzzing technology that is optimized for Microservice environments and implemented as RockFuzz. The identified key challenges are addressed through mechanisms to repeat tests with mocking data, re-executing tests mocking-assisted seed replay, seed refresh and distributed log tracing. The evaluation on a large case study from the finance sector with hundreds of microservices and two further scenarios could confirm that the contributions are suitable to identify many vulnerabilities.

Strengths
---------
* The paper proposes a novel approach for fuzzing in microservice environments.
* The paper outlines the domain's challenges and how the solution addresses them well.
* The evaluation is based on a big case study.

Weaknesses
----------
* Alternative solutions are neglected, the overall design process is only presented in its results.
* The discussion of related work is shallow.
* The structure of the evaluation and results presentation.

Comments for authors
--------------------
For many concrete design and parameter decisions, e.g., the seed management, the results are explained; however, there is not much detail in how these decisions were taken, which would be needed to apply the approach to other scenarios.

The evaluation presentation could be massively improved by making the research objectives/questions explicit and clearly separating question, setup, execution, results, and their discussion. 

The RockFuzz architecture diagram is hard to read due to the amount and placement of the arrows. The authors should try to improve it by aggressively trying to merge and optimize placement.

336-338: Such statements should be backed by evidence/citation

Questions for authors’ response
-------------------------------
1. What are the rationals behind the core design decisions and which assumptions and limitations do they imply?



Review #409C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper presents RockFuzz, an industrial fuzzing framework for microservice applications. RockFuzz targets one service at a time, and handles external dependencies on other services using mocking-assisted seed replay and periodic seed refresh to balance accuracy of results with performance. Distributed tracing is used to enable complete code coverage collection and to overcome communication overhead between the fuzzer and the service under test. RockFuzz supports 3 application use cases: regular fuzzing, iteration testing and taint verification. Results from deployment in a financial company indicate RockFuzz's effectiveness and maturity, as it has found 1615 vulnerabilities in regular fuzzing and 600+ security risks in taint verification, over a period of 3 months.

Strengths
---------
+ Significant and relevant problem
+ The technique handles practical aspects of fuzzing in modern microservice applications
+ The paper presents 3 different application use cases and their results 
+ The paper presents impressive results from field deployment in a large financial company

Weaknesses
----------
- The motivation for the work is not clearly explained
- Novelty is unclear, despite the claim to be the first fuzzing framework for microservices
- The framework is not systematically evaluated nor compared to SOTA techniques, but rather results from field deployment are reported as in an experience report
- Results are from 84 services out of 3000+, it is not explained how and why they were chosen 
- There are some presentation issues
- The framework, the case study application and the related data are not available

Comments for authors
--------------------
I found this paper very interesting. It handles an important and relevant problem to the practice, that of fuzzing of Cloud applications, and unveils practical challenges and bottlenecks in real world application of fuzzing. RockFuzz suggests solutions to overcome these challenges and delivers impressive field results, though it was very partially applied to the FinTech company (84 out of 3000+ services), and detailed results are presented for only 10 services. It would be beneficial to explain why and how the 84 services were chosen, and make their full results available. I also liked the 3 different application use cases presented, and how the technique was tweaked for each of them. 

Despite these positive points, I have two main concerns about this work. My first concern is regarding motivation and novelty. I wasn't convinced by the authors motivation for a dedicated fuzzer for microservices. The paper starts with a very strong statement that microservices "makes all the existing fuzzers invalid when used to fuzz microservices", but the authors then don't really deliver on this statement by explaining why they are invalidated. In the introduction, the challenges are only briefly mentioned and not explained at all. Only later they become clear. The authors also don't explain how existing fuzzers work, which is a gap in their background and challenges section. Following that, it is unclear why existing tools such as AFL and others cannot be applied to each service separately, just like RockFuzz. The technical novelty then also becomes unclear. I argue that challenges 1 and 2 exist at least partially also in monolithic applications. To the very least, system dependencies and internal dependencies precede microservices by decades, and hence must have been handled also by existing fuzzers. As for handling external dependencies, I understand that when service A calls service B this might result in inconsistency if service B has changed, but what is the real impact of ignoring this case and letting the fuzzer use current results like AFL would do? this has been deemed infeasible without actually being evaluated. Regarding challenge 3, overcoming communication overhead and achieving a complete view of the system are mostly engineering tasks, and the use of distributed tracing is prevalent in Cloud applications for such purposes. Complete code coverage is also reported for example by a dozen of existing REST API test generation tools, so the novel contribution for challenge 3 needs to be further clarified. 

My second concern is regarding the evaluation. It simply reports partial field results from 3 months' deployment, without describing (1) the system under test, (2) the choice of 84 services from 3000+ and the choice of 10 services to present in Table 2 from 84, (3) experimental setup, and (4) research questions. Most importantly, RockFuzz is not compared to SOTA techniques for fuzzing. The only exception is column #TO in Table 2, which presents the cost (in milliseconds) of fuzzing without decoupling modules, and tagged as "non-blocking implementation of monolithic fuzzers". However, monolithic fuzzers don't necessarily need to be applied to the whole system, they could be applied to each service separately. Moreover, the cost in runtime is not the only aspect to consider when comparing to "monolithic fuzzers". Other aspects such as coverage achieved and vulnerabilities found should be considered as well in the comparison.

There are also presentation issues (some are mentioned in the "more comments" list below). Specifically, the presentation mixes conceptual technique details with implementation details, e.g., Section 3 describing the framework operation, it delves into low level implementation details: "OpenTracing [37] is used to automatically instrument the target Apps by attaching Java agents [3] which perform Java bytecode instrumentation at runtime". This is the first mention of Java and I deduce that the framework supports Java only?. The presentation also mixes implementation with evaluation description in Section 5. For example, Section 5.1.4 already refers to the evaluation, hence should be moved from section 5.1 which is about implementation.

To summarize, I think that this work could have been a strong contribution as an experience report. Unfortunately, as a research paper, it doesn't pass the bar for me in terms of technical contribution nor in terms of expected evaluation.

More comments:
- Inconsistent terminology for a service: service/microservice/App/component
- "especially when the dependent Apps may evaluate" - what does this mean? dependent apps may evaluate what? 
- At the end of the introduction in the summary of contribution, the authors state ""Specially, RockFuzz can greatly save CPU resources without loss of coverage". This is the first time a statement about RockFuzz's performance is made. It should be referred to and explained earlier. 
- "and there exists a value of this mocking point in the mocks database" - what does this value represent? an identifier of the mocking point? a seed according to which inputs are chosen? this is unclear
- Related work briefly describes SOTA techniques, but doesn't position RockFuzz against it, so it is unclear how it differentiates from existing work.
- There is a typo in Conclusion Section:  relay -> replay
- There is no future work description by the authors

Questions for authors’ response
-------------------------------
1. What prevents running existing "monolithic" fuzzers on each service separately, then combining results as RockFuzz does? is it just external dependencies on services with high release rate or are there other inhibitors as well?
2. Why was RockFuzz applied to only 84 services out of 3000+? how were these services chosen?



Review #409D
===========================================================================

Metareview
----------
Thank you for submitting your work to ISSTA 2023. The reviewers agreed that while the paper targets an important problem, there are several issues with the current version. The presentation could be significantly improved and the contributions could be more clearly described. One key missing component is a discussion of prior work using existing fuzzers for microservices and how this paper's contribution is an improvement over them.
We hope the reviews will help improve your paper for future submissions!

Decision
--------
1. Reject
